Scalable Consistency Training for Graph Neural Networks via Self-Ensemble Self-Distillation

Consistency training is a popular method to improve deep learning models in computer vision and natural language processing. Graph neural networks (GNNs) have achieved remarkable performance in a variety of network science learning tasks, but to date no work has studied the effect of consistency training on large-scale graph problems. GNNs scale to large graphs by minibatch training and subsample node neighbors to deal with high degree nodes. We utilize the randomness inherent in the subsampling of neighbors and introduce a novel consistency training method to improve accuracy. For a target node we generate different neighborhood expansions, and distill the knowledge of the average of the predictions to the GNN. Our method approximates the expected prediction of the possible neighborhood samples and practically only requires a few samples. We demonstrate that our training method outperforms standard GNN training in several different settings, and yields the largest gains when label rates are low.

==> tables/arxiv_consistency_multiple_models.tex <==
\begin{table*}[htbp]
\caption{ogbn-arxiv Consistency Training Results, Inductive Setting}
\begin{center}
\begin{tabular}{|c|r|r|r|r|}
\hline
\textbf{Model} & \textbf{Label Rate} & \textbf{Layers} & {\bf Baseline Test Acc } & {\bf Consistency Test Acc }  \\\hline
GCN & 55.0 & 3 & 69.67$\pm$0.41 & 70.12$\pm$0.15 \\\hline
GAT & 55.0 & 3 & 70.33$\pm$0.19 & 70.72$\pm$0.31  \\\hline
GCN & 55.0 & 2 & 68.42$\pm$0.30 & 69.19$\pm$0.14\\\hline
GAT & 55.0 & 2 & 69.48$\pm$0.34 & 69.61$\pm$0.09 \\\hline
GCN & 5.5 & 3 & 66.10$\pm$0.44 & 68.07$\pm$0.41 \\\hline
GAT & 5.5 & 3 & 65.81$\pm$0.92 & 67.45$\pm$0.26 \\\hline
GCN & 5.5 & 2 & 64.71$\pm$0.48 & 66.04$\pm$0.36 \\\hline
GAT & 5.5 & 2 & 65.23$\pm$0.48 & 65.99$\pm$0.54\\\hline
\end{tabular}
\label{tab: arxiv consistency multiple models}
\end{center}
\end{table*}

==> tables/consistency_baseline_se.tex <==
\begin{table*}[htbp]
\caption{ogbn-arxiv consistency training results, inductive setting}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Label Rate} & \textbf{Layers} & {\bf Baseline Test Acc } & {\bf Consistency Test Acc }  \\\hline
GCN & 55 & 3 & 69.67$\pm$0.41 & 70.51$\pm$0.27 \\\hline
GAT & 55 & 3 & 70.33$\pm$0.19 & 70.72$\pm$0.31  \\\hline
GCN & 55 & 2 & 68.42$\pm$0.30 & 69.19$\pm$0.14\\\hline
GAT & 55 & 2 & 69.48$\pm$0.34 & 69.61$\pm$0.09 \\\hline
GCN & 5.5 & 3 & 66.10$\pm$0.44 & 68.07$\pm$0.41 \\\hline
GAT & 5.5 & 3 & 65.81$\pm$0.92 & 67.45$\pm$0.26 \\\hline
GCN & 5.5 & 2 & 64.71$\pm$0.48 & 66.04$\pm$0.36 \\\hline
GAT & 5.5 & 2 & 65.23$\pm$0.48 & 65.99$\pm$0.54\\\hline
\end{tabular}
\label{tab: arxiv consistency multiple models}
\end{center}
\end{table*}

==> tables/products_consistency_multiple_models.tex <==
\begin{table*}[htbp]
\caption{ogbn-products Consistency Training Results, Transductive Setting, Fanout-5}
\begin{center}
\begin{tabular}{|c|r|r|r|r|}
\hline
\textbf{Model} & \textbf{Label Rate} & \textbf{Layers} & {\bf Baseline Test Acc } & {\bf Consistency Test Acc }  \\\hline
GCN & 8.0 & 3 & 79.61$\pm$0.26   & 79.88$\pm$0.22 \\\hline
GAT & 8.0 & 3 & 79.70$\pm$0.60  & 80.04$\pm$0.48  \\\hline
GCN & 0.8 & 3 & 76.01$\pm$0.20 & 77.64$\pm$0.60  \\\hline
GAT & 0.8 & 3 & 75.96$\pm$0.69 & 77.89$\pm$0.76 \\\hline
\end{tabular}
\label{tab: products consistency multiple models}
\end{center}
\end{table*}

==> tables/products_transductive_fanout_5.tex <==
\begin{table*}[htbp]
\caption{Products, Ensemble vs Self-Ensembling, GCN-2 Fanout-5}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c}
\hline
\textbf{Number}&\multicolumn{5}{|c|}{\textbf{Number of Models}} \\
\cline{2-6}\textbf{of Views} & 1 & 2 & 3 & 4 & 5 \\
\hline
1 & 76.24$\pm$0.43 & 76.77$\pm$0.29 & 76.8$\pm$0.23 & 76.81$\pm$0.2 & 76.75$\pm$0.27 \\\hline
2 & 77.06$\pm$0.48 & 77.07$\pm$0.31 & 77.54$\pm$0.2 & 77.3$\pm$0.14 & 77.49$\pm$0.06 \\\hline
3 & 77.04$\pm$0.39 & 77.32$\pm$0.31 & 77.52$\pm$0.18 & 77.7$\pm$0.18 & 77.69$\pm$0.21 \\\hline
4 & 77.45$\pm$0.5 & 77.36$\pm$0.21 & 77.81$\pm$0.24 & 77.66$\pm$0.2 & 77.57$\pm$0.13  \\\hline
5 & 77.33$\pm$0.38 & 77.59$\pm$0.28 & 77.84$\pm$0.27 & 77.83$\pm$0.18 & 77.95$\pm$0.13  \\\hline
\end{tabular}
\label{tab: products transductive fanout 5}
\end{center}
\end{table*}



==> tables/reddit_consistency_multiple_models.tex <==
\begin{table*}[htbp]
\caption{Reddit Consistency Training Results, Inductive Setting, Fanout-20}
\begin{center}
\begin{tabular}{|c|r|r|r|r|}
\hline
\textbf{Model} & \textbf{Label Rate} & \textbf{Layers} & {\bf Baseline Test Acc } & {\bf Consistency Test Acc }  \\\hline
GCN & 66.0 & 2 & 96.13$\pm$0.04   & 95.90$\pm$0.01 \\\hline
GAT & 66.0 & 2 & 95.95$\pm$0.09 & 96.20$\pm$0.02  \\\hline
GCN & 6.6 & 2 & 94.74$\pm$0.04  & 95.28$\pm$0.05  \\\hline
GAT & 6.6 & 2 & 95.04$\pm$0.11 & 95.82$\pm$0.07 \\\hline
\end{tabular}
\label{tab: reddit consistency multiple models}
\end{center}
\end{table*}

==> tables/reddit_gcn_inductive_se.tex <==
\begin{table*}[htbp]
\caption{Reddit test accuracy, Ensemble vs Self-Ensembling, Inductive GCN-2 Fanout-20}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c}
\hline
\textbf{Number}&\multicolumn{5}{|c|}{\textbf{Number of Models}} \\
\cline{2-6}\textbf{of Views} & 1 & 2 & 3 & 4 & 5 \\
\hline
1 & 96.15$\pm$0.06 & 96.32$\pm$0.02 & 96.40$\pm$0.01 & 96.35$\pm$0.02 & 96.42$\pm$0.05 \\ \hline
2 & 96.26$\pm$0.04 & 96.46$\pm$0.02 & 96.53$\pm$0.05 & 96.54$\pm$0.02 & 96.55$\pm$0.04 \\ \hline
3 & 96.33$\pm$0.04 & 96.51$\pm$0.05 & 96.56$\pm$0.03 & 96.55$\pm$0.04 & 96.57$\pm$0.04 \\ \hline
4 & 96.43$\pm$0.02 & 96.54$\pm$0.02 & 96.56$\pm$0.01 & 96.56$\pm$0.04 & 96.58$\pm$0.02 \\ \hline
5 & 96.37$\pm$0.04 & 96.55$\pm$0.03 & 96.59$\pm$0.04 & 96.62$\pm$0.04 & 96.62$\pm$0.01 \\ 
\hline
\end{tabular}
\label{tab: reddit inductive self-ensemble}
\end{center}
\end{table*}


